G\'eom\'etrie anab\'elienne temp\'er\'ee

The tempered fundamental group of a p-adic analytic variety classifies \'etale coverings that become topological coverings (for the Berkovich topology) after finite \'etale base change. I study what can be recovered from the tempered fundamental group. In particular, I prove that, for a Mumford curve, one can recover the metric of the graph of the stable reduction from the tempered fundamental group. I also study how the tempered fundamental group behaves along the fibers of a fibration.

==> chap3.tex <==

\chapter{Propriétés anabéliennes du groupe fondamental tempéré} 
\input{metric}
 
